Power Optimization for Network Localization

Reliable and accurate localization of mobile objects is essential for many applications in wireless networks. In range-based localization, the position of the object can be inferred using the distance measurements from wireless signals exchanged with active objects or reflected by passive ones. Power allocation for ranging signals is important since it affects not only network lifetime and throughput but also localization accuracy. In this paper, we establish a unifying optimization framework for power allocation in both active and passive localization networks. In particular, we first determine the functional properties of the localization accuracy metric, which enable us to transform the power allocation problems into second-order cone programs (SOCPs). We then propose the robust counterparts of the problems in the presence of parameter uncertainty and develop asymptotically optimal and efficient near-optimal SOCP-based algorithms. Our simulation results validate the efficiency and robustness of the proposed algorithms.

==> Bios/MoeWinIEEEBio-V39.tex <==
%{\bf Moe Z. Win} (S'85-M'87-SM'97-F'04) received 
%the B.S. degree ({\em magna cum laude}) from Texas A\&M University, College Station, in 1987, and 
%the M.S. degree from the University of Southern California (USC), Los Angeles, in 1989, both in Electrical Engineering. 
%As a Presidential Fellow at USC, he received both
%an M.S. degree in Applied Mathematics and the Ph.D. degree in Electrical Engineering in 1998.
%He has been named a Distinguished Alumnus of Mountain View College.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%	E D U C A T I O N
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
(S'85-M'87-SM'97-F'04) 
received 
	both the Ph.D.\ in 
		\switchAtwo{Electrical Engineering}
				{Electrical Engineering (under the supervision of Professor Robert A.\ Scholtz)}
	and the M.S.\ in 
		\switchAtwo{Applied Mathematics}
				{Applied Mathematics (under the supervision of Professor Solomon W.\ Golomb)}
		as a Presidential Fellow at the University of Southern California (USC) in 1998.
He received the M.S.\ in Electrical Engineering from USC in 1989 
	and the B.S.\ ({\em magna cum laude}) in Electrical Engineering from Texas A\&M University in 1987.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%	E X P E R I E N C E
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
He is a Professor at the Massachusetts Institute of Technology (MIT)
and the founding director of the Wireless Communication and Network Sciences Laboratory. 
%Dr.\ Win is a Professor at the Laboratory for Information
%\& Decision Systems (LIDS), Massachusetts Institute of Technology (MIT).
%%Dr.\ Win joined the Laboratory for Information and Decision Systems (LIDS)
%%%and the Department of Aeronautics and Astronautics,
%%at the Massachusetts Institute of Technology in 2002, where he is an Associate Professor.
Prior to joining MIT, he was with AT\&T Research Laboratories for five years 
and with the Jet Propulsion Laboratory for seven years.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%	R E S E A R C H	I N T E R E S T S
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
His research encompasses fundamental theories, algorithm design, and
experimentation for a broad range of real-world problems.
%His research encompasses developing fundamental theories, designing algorithms, and
%conducting experimentation for a broad range of real-world problems.
%His main research interests are the applications of mathematical and
%statistical theories to communication, detection, and estimation problems.
His current research topics include
%	location-aware networks, 
%	intrinsically secure wireless networks,
%	aggregate interference in heterogeneous networks,
	network localization and navigation, 
	network interference exploitation, 
	intrinsic wireless secrecy,
	adaptive diversity techniques,
		\switchBtwo{and ultra-wide bandwidth systems.}
				{ultra-wide bandwidth systems,
			%	time-varying channels, 
				optical transmission systems, 
				and 
				space communications systems.}
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%	M A J O R		R E C O G N I T I O N S	
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Professor Win is 
	an elected Fellow of the AAAS, the IEEE, and the IET, 
	and was an IEEE Distinguished Lecturer.
%	elected Fellow of the IEEE, cited for ``contributions to wideband wireless transmission.''
He was honored with two IEEE Technical Field Awards: 
	the IEEE Kiyo Tomiyasu Award (2011) 
		\switchBtwo{and}
				{for ``fundamental contributions to high-speed reliable communications over optical and wireless channels''  and}
	the IEEE Eric E. Sumner Award 
		\switchBtwo{(2006, jointly with R.\ A.\ Scholtz).}
				{(2006, jointly with R.\ A.\ Scholtz) for ``fundamental contributions to high-speed reliable communications over optical and wireless channels.''}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%	P A P E R		A W A R D S	
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Together with students and colleagues, his papers have received numerous awards, including
	\switchBtwo{the IEEE Communications Society's Stephen O.\ Rice Prize (2012),
			the IEEE Aerospace and Electronic Systems Society's M.\ Barry Carlton Award (2011),
			the IEEE Communications Society's Guglielmo Marconi Prize Paper Award (2008),
    			and the IEEE Antennas and Propagation Society's Sergei A.\ Schelkunoff Transactions Prize Paper Award (2003).}
			{the IEEE Communications Society's Stephen O.\ Rice Prize (2012),
			the IEEE Communications Society's William R.\ Bennett Prize (2012),
			the IEEE Communications Society's Fred W.\ Ellersick Prize (2012),
			the IEEE Communications Society's Leonard G.\ Abraham Prize (2011),
			the IEEE Aerospace and Electronic Systems Society's M.\ Barry Carlton Award (2011),
			the IEEE Communications Society's Guglielmo Marconi Prize Paper Award (2008),
    			and the IEEE Antennas and Propagation Society's Sergei A.\ Schelkunoff Transactions Prize Paper Award (2003).}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%	F E L L O W S H I P S
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Highlights of his international research and education collaborations include
%Highlights of his worldwide educational and research collaborations are
Highlights of his international scholarly initiatives are
	the Copernicus Fellowship (2011),
	the Royal Academy of Engineering Distinguished Visiting Fellowship (2009),
%	Institute of Advanced Study Natural Sciences and Technology Fellowship (2004),
	and
	the Fulbright
		\switchBtwo{Fellowship (2004).}
				{Foundation Senior Scholar Lecturing and Research Fellowship (2004).}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%	O T H E R		R E C O G N I T I O N S
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Other recognitions include
	\switchBtwo{the International Prize for Communications Cristoforo Colombo (2013),
				the {\it Laurea Honoris Causa} from the University of Ferrara (2008),	
				the Technical Recognition Award of the IEEE ComSoc Radio Communications Committee (2008),
        				and the U.S. Presidential Early Career Award for Scientists and Engineers (2004).}	
			{the International Prize for Communications Cristoforo Colombo (2013),
				the Outstanding Service Award of the IEEE ComSoc Radio Communications Committee (2010),
				the {\it Laurea Honoris Causa} from the University of Ferrara, Italy (2008),
				the Technical Recognition Award of the IEEE ComSoc Radio Communications Committee (2008),
        				the Wireless Educator of the Year Award (2007),
				the U.S. Presidential Early Career Award for Scientists and Engineers (2004), 
				the AIAA Young Aerospace Engineer of the Year (2004),
				and
				the Office of Naval Research Young Investigator Award (2003).}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%	E L E C T E D		P O S I T I O N S
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Dr.\ Win is an elected Member-at-Large on the IEEE Communications Society Board of Governors (2011--2013).
%Professor Win has been actively involved in various aspects of IEEE. 
%His active involvement in IEEE includes 
He was
    the Chair (2004--2006) and Secretary (2002--2004) for
        the Radio Communications Committee of the IEEE Communications Society.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%	C O N F E R E N C E S
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Professor Win has been actively involved in organizing and chairing
%%sessions, and has served as a member of the Technical Program Committee in
%a number of international conferences. 
\switchBtwo{Over the last decade, he has organized and chaired numerous international conferences.} 
		{He served as
			the Technical Program Chair for
				the IEEE Wireless Communications and Networking Conference (2009),
				the IEEE Conference on Ultra Wideband (2006),
				the IEEE Communication Theory Symposia of ICC (2004) and Globecom (2000),
				 and
				the IEEE Conference on Ultra Wideband Systems and Technologies (2002);
			Technical Program Vice-Chair for
				the IEEE International Conference on Communications (2002); and
			the Tutorial Chair for
				ICC (2009) and
				the IEEE Semiannual International Vehicular Technology Conference (Fall 2001).}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%	E D I T O R I A L S
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
He is currently
	an Editor-at-Large for the 
	{\scshape IEEE Wireless Communications Letters}
and is serving on 
	the Editorial Advisory Board for the 
	{\scshape IEEE Transactions on Wireless Communications}.
% He served as Editor (2006--2012) for
% 	\switchBtwo{the {\scshape IEEE Transactions on Wireless Communications},
% 				and as 
% 				Area Editor (2003--2006) and Editor (1998--2006)
% 				for the {\scshape IEEE Transactions on Communications}.}      	
% 			  {the {\scshape IEEE Transactions on Wireless Communications}.
% 				He also served as the
% 	    			Area Editor for {\em Modulation and Signal Design} (2003--2006),
% 	    			Editor for {\em Wideband Wireless and Diversity} (2003--2006), and
% 	    			Editor for {\em Equalization and Diversity} (1998--2003),
% 	        			all for the {\scshape IEEE Transactions on Communications}.}
% He was Guest-Editor
%         for the
%         {\scshape Proceedings of the IEEE}
% 		\switchBtwo{(2009)}
% 				{(Special Issue on UWB Technology \& Emerging Applications -- 2009)} and
%         {\scshape IEEE Journal on Selected Areas in Communications}
%         		 \switchBtwo{(2002).}
% 		 		{(Special Issue on Ultra\thinspace-Wideband Radio in Multiaccess Wireless Communications  -- 2002).}

                
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newpage
%\vspace{0.6cm} {\large
%
%\centerline{\bf Please Note}
%
%The electronic version of the photograph for Moe Win is enclosed in the
%accompanying diskette.
%
%Please contact me if this is not satisfactory.  I can be reached at Tel: (732)-687-8113, Fax:
%(617)-253-3578 or e-mail: {\tt moewin@mit.edu}. }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Professor Win received
%%    the IEEE Communications Society Best Student Paper Award at the Fourth Annual IEEE
%%        NetWorld+Interop'97 Conference in 1997,
%%    the International Telecommunications Innovation Award from Korea Electronics Technology Institute in 2002,
%    a Young Investigator Award from the Office of Naval Research
%%    in 2003,
%    and
%    the IEEE Antennas and Propagation Society Sergei A. Schelkunoff Transactions Prize Paper Award in 2003.
%In 2004, Dr. Win was named
%        Young Aerospace Engineer of the Year by AIAA,
%    and garnered
%        the Fulbright Foundation Senior Scholar Lecturing and Research Fellowship,
%        the Institute of Advanced Study Natural Sciences and Technology Fellowship,
%%        the Outstanding International Collaboration Award from the Industrial Technology Research Institute of Taiwan,
%        and
%        the Presidential Early Career Award for Scientists and Engineers from the United States White House.
%He was honored with
%%        the Lifetime Achievement Award from the People of Bangladesh in 2006,
%%        and in that same year received
%%        the IEEE Eric E. Sumner Award
%%        ``for pioneering contributions to ultra-wide band communications science and
%%        technology.''
%        the 2006 IEEE Eric E. Sumner Award, an IEEE Technical Field Award,
%        ``for pioneering contributions to ultra-wide band communications science and
%        technology.''
%Professor Win is an IEEE Distinguished Lecturer and
%        elected Fellow of the IEEE, cited ``for contributions to wideband wireless transmission.''

